Bayesian Nonparametric Models for Biomedical Data Analysis

In this dissertation, we develop nonparametric Bayesian models for biomedical data analysis. In particular, we focus on inference for tumor heterogeneity and inference for missing data. First, we present a Bayesian feature allocation model for tumor subclone reconstruction using mutation pairs. The key innovation lies in the use of short reads mapped to pairs of proximal single nucleotide variants (SNVs). In contrast, most existing methods use only marginal reads for unpaired SNVs. In the same context of using mutation pairs, in order to recover the phylogenetic relationship of subclones, we then develop a Bayesian treed feature allocation model. In contrast to commonly used feature allocation models, we allow the latent features to be dependent, using a tree structure to introduce dependence. Finally, we propose a nonparametric Bayesian approach to monotone missing data in longitudinal studies with non-ignorable missingness. In contrast to most existing methods, our method allows for incorporating information from auxiliary covariates and is able to capture complex structures among the response, missingness and auxiliary covariates. Our models are validated through simulation studies and are applied to real-world biomedical datasets.

==> Makediss <==
#!/bin/sh
#
# Makediss
#
# A Bourne shell script file to compile the dissertation template.
# The test of exit code after the first latex command causes
# execution of the shell script to stop if there were unresolved
# errors (so one will not have to repeat the same steps four more
# times before the shell script ends).
#
#	22 Jul 2001		Craig McCluskey
# 
#	23 Sep 2001		Craig McCluskey
#		- added checking for existing gv process.
#
#	04 Oct 2001		Craig McCluskey
#		- added removing of extra files from previous run.
#
#	09 Oct 2001		Craig McCluskey
#		- added comments.
#	29 Nov 2001		Craig McCluskey
#		- added code to compare existing utdiss2.sty to
#		  the latest style file ($STY) in case someone
#		  has gotten a new style file and not removed the
#		  copy of the old one.
#	07 Dec 2001		Craig McCluskey
#		- made viewing the PostScript the default after
#		  generating it.
#	16 Dec 2001		Craig McCluskey
#		- added echo commands of each run of a command.
#	23 Dec 2001		Craig McCluskey
#		- added gv options media and noresize.
#	16 Jan 2002		Craig McCluskey
#		- added -t option to dvips to force using
#		  of letter-sized paper.
#	13 Mar 2002		Craig McCluskey
#		- changed compare of utdiss2.sty to ask use if
#		  he wants to update.
#		- changed rm -f $DISS.aux to rm -f *.aux to remove
#		  auxillary files for chapters, too.
#		- added clear.
#		- removed echo "utdiss2 already exists."
#		- added test for existence of $STY.
#		- made exit values increase for each subsequent exit.
#	25 Aug 2002		Craig McCluskey
#		- changed STY to utdiss2-05.sty.
#

DISS="./disstemplate"	# Change this to the name of your
			# dissertation file.

STY="utdiss2-05.sty"

# Remove working files from last run.
#
rm -f $DISS.log \
	*.aux \
	$DISS.bbl \
	$DISS.blg \
	$DISS.dvi \
	$DISS.idx \
	$DISS.ilg \
	$DISS.ind \
	$DISS.lof \
	$DISS.log \
	$DISS.lot \
	$DISS.ps \
	$DISS.toc	2>/dev/null

# Clear the screen.
#
clear

# Make sure the latest version of the style file exists.
#
if test ! -e $STY
  then
    echo ""
    echo "	$STY does not exist!"
    echo ""
    exit 1
fi

# Copy the latest version of the utdiss2 style file to utdiss2.sty.
#
if test -e utdiss2.sty
  then
    cmp utdiss2.sty $STY > /dev/null 2>&1
    retval="$?"
    if test $retval -ne 0
      then
	echo ""
	echo ""
	echo "	$STY and utdiss2.sty are different."
	echo ""
	echo -n "Over-write utdiss2.sty with $STY ? (y/<return>)"
	read reply
	if test "$reply" = "y"
	  then
	    cp -fa $STY utdiss2.sty
	    echo ""
	    echo "	utdiss2.sty over-written."
	    echo ""
	  else
	    echo ""
	    echo "	utdiss2.sty NOT over-written."
	    echo ""
	fi
	echo ""
	sleep 1
    fi
  else
    cp -a $STY utdiss2.sty
fi


# Run latex, bibtex, and makeindex to create the output file ($DISS.dvi)
#
echo ""
echo "	First run of LaTeX ..."
echo ""
latex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 2
	fi
echo ""
echo "	Run of BibTeX ..."
echo ""
bibtex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 3
	fi
echo ""
echo "	Second run of LaTeX ..."
echo ""
latex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 4
	fi
echo ""
echo "	Third run of LaTeX ..."
echo ""
latex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 5
	fi
echo ""
echo "	Run of makeindex ..."
echo ""
makeindex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 6
	fi
echo ""
echo "	Fourth run of LaTeX ..."
echo ""
latex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 7
	fi
echo ""
echo "	Fifth and last run of LaTeX ..."
echo ""
latex $DISS
exitcode="$?"
	if test $exitcode -ne 0
	  then
	    exit 8
	fi

# Make the postscript file from the .dvi file. The t option forces
# dvips to make the postscript file for letter (8.5 x 11) size paper.
#
dvips -t letter $DISS -o


# If the user is not looking at the postscript file already, ask him
# if he wants to. If so, start GhostView.
#
echo ""
echo ""
echo ""
echo ""
echo ""
echo ""
echo 

# ps -ef 2>/dev/null | grep -v grep | grep "gv" \
# 			| grep "$DISS.ps" > /dev/null 2>&1

ps -eo cmd 2>/dev/null | grep -v grep | grep "gv" \
			| grep "$DISS.ps" > /dev/null 2>&1
retval="$?"
if test $retval -ne 0
  then
    echo 
    echo "	View Postscript? <return/n> "
    read reply
    if test "$reply" != "n"
      then
        gv $DISS.ps &
        # gv -media letter -noresize $DISS.ps &
    fi
  else
    echo 
fi

